Geometric convergence of elliptical slice sampling

For Bayesian learning, given likelihood function and Gaussian prior, the elliptical slice sampler, introduced by Murray, Adams and MacKay 2010, provides a tool for the construction of a Markov chain for approximate sampling of the underlying posterior distribution. Besides of its wide applicability and simplicity its main feature is that no tuning is necessary. Under weak regularity assumptions on the posterior density we show that the corresponding Markov chain is geometrically ergodic and therefore yield qualitative convergence guarantees. We illustrate our result for Gaussian posteriors as they appear in Gaussian process regression, as well as in a setting of a multi-modal distribution. Remarkably, our numerical experiments indicate a dimension-independent performance of elliptical slice sampling even in situations where our ergodicity result does not apply.

==> sections/numerical_experiments.tex <==
\section{Numerical experiments}
\label{sec:numerical-experiments}

In the original paper \cite{murray2010elliptical} the authors have already
performed several numerical experiments, in particular: Gaussian regression,
Gaussian process classification and Log Gaussian Cox process.
In this section we expand this list by providing the results of sampling w.r.t.
to a density of the so-called \textit{double banana} form. Moreover, we compare
the Elliptical Slice Sampler with other MCMC methods in terms of effective
sample size.

\subsection{Double banana}
We sample w.r.t. the two-dimensional distribution
\[
    \mu(\d x)
    =
    \exp
    (
        -|\alpha - \log F(x)|
    )
    \d x,
    \qquad
    x \in \mathbb{R}^2
\]
with $\alpha = 5$ and a scalar logarithmic Rosenbrock function
\[
    F(x)
    =
    \log
    \left(
        (1 - x_1)^2 + 100(x_2 - x_1^2)^2
    \right).
\]
Using the two-dimensional standard Gaussian reference measure
$\mu_0 = \mathcal{N}(0, I_2)$ the measure $\mu$ corresponds e.g. to the function
\[
    \rho(x)
    =
    \exp
    \left(
        \frac{1}{2}\|x\|^2
        -|\alpha - \log F(x)|
    \right),
    \qquad
    x \in \mathbb{R}^2
\]
from \eqref{equ:densities}.
The samples w.r.t. the measure $\mu$ generated by the Elliptical Slice Sampler
are presented in the histogram on the Figure~\ref{fig:double-banana}.
In this example the first $10^5$ steps of the algorithm were considered as
burn-in and were removed from the sample list.
\begin{figure}
    \begin{center}
        \includegraphics[width=0.48\textwidth]{pics/double_banana.pdf}
    \end{center}
    \caption
    {
        Two-dimensional histogram of $10^6$ samples generated by the Elliptical
        Slice Sampler for the \textit{double banana} example.
    }
    \label{fig:double-banana}
\end{figure}

\subsection{Comparison with other MCMC algorithms}
We performed numerical experiments and compared Elliptical Slice Sampler with
several other MCMC methods in terms of effective sample size in different
dimensions.
Before presenting the results we provide some basics for the understanding of
numerical experiments.

As a metric for comparison of different MCMC algorithms we consider and estimate
the effective sample size
\[
    \mathrm{ESS}
    =
    \mathrm{ESS}(n, f, (X_k)_{k\in\mathbb{N}})
    =
    n
    \left(
        1 + 2 \sum_{k=0}^\infty \gamma_f(k)
    \right)^{-1}.
\]
Here $n$ is the number of samples taken from Markov chain
$(X_k)_{k\in\mathbb{N}}$, f is the function of interest and $\gamma_f$ denotes
the autocorrelation function
\[
    \gamma_f(k)
    =
    \mathrm{Corr}(f(X_{n_0}), f(X_{n_0+k})),
\]
where $n_0$ denotes the so called burn-in number.
We perform the experiments with $\mu_0 = \mathcal{N}(0, I)$ for the density
\[
    \rho(x)
    =
    \exp
    \left(
        \|x\|
    \right),
    \qquad
    x \in \mathbb{R}^d,
\]
which corresponds to the \textit{volcano} measure (see
Figure~\ref{fig:volcano_denisty})
\[
    \mu (\d x)
    =
    \exp
    \left(
        \|x\| - \frac{1}{2} \|x\|^2
    \right)
    \d x,
    \qquad
    x \in \mathbb{R}^d,
\]
and for the function of interest $f(x) = \log(1 + \|x\|)$.
\begin{figure}
	\begin{center}
		\includegraphics[width=0.48\textwidth]{pics/volcano_density.pdf}
	\end{center}
	\caption{Density of two-dimensional \textit{volcano} measure.}
	\label{fig:volcano_denisty}
\end{figure}
\begin{figure}
	\begin{center}
		\includegraphics[width=0.48\textwidth]{pics/effective-sample-size.pdf}
	\end{center}
    \caption
    {
        Effective sample size for different MCMC algorithms depending on the
        dimension of the space.
    }
	\label{fig:ESS}
\end{figure}
In our simulations each algorithm started at $0$, performed firstly $n_0=10^5$
steps (as burn-in) and then saved the next $n=10^6$ steps.
We ran all algorithms for the dimensions $30, 100, 300$ and $1000$.
We provide the graph of effective sample size depending on dimension $d$
(see Figure~\ref{fig:ESS}).
Both Metropolis algorithms (Random Walk Metropolis and Preconditioned
Crank--Nicolson) were tuned to have the acceptance probability about $0.25$.
What we can conclude from the picture is on one hand that the Simple Slice
Sampler and the Random Walk Metropolis (RWM) depend strongly on the dimension in
terms of effective sample size.
On the other hand, Elliptical Slice Sampler and the Preconditioned
Crank--Nicolson (pCN) show dimension-independent and overall better behaviour.
At this point we also emphasize that the Elliptical Slice Sampler does not need
to be tuned in comparison to the pCN in spite of having similar performance.
However, the price of the privilege not to tune the algorithm is the need of
evaluating the function $\rho$ more times within one step of the algorithm.
In our example the function $\rho$ was evaluated on average $1.5$ times per one
step of the Elliptical Slice Sampler.
